Hybrid Iterative Linear Quadratic Estimation: Optimal Estimation for Hybrid Systems

In this paper we present Hybrid iterative Linear Quadratic Estimation (HiLQE), an optimization based offline state estimation algorithm for hybrid dynamical systems. We utilize the saltation matrix, a first order approximation of the variational update through an event driven hybrid transition, to calculate gradient information through hybrid events in the backward pass of an iterative linear quadratic optimization over state estimates. This enables accurate computation of the value function approximation at each timestep. Additionally, the forward pass in the iterative algorithm is augmented with hybrid dynamics in the rollout. A reference extension method is used to account for varying impact times when comparing states for the feedback gain in noise calculation. The proposed method is demonstrated on an ASLIP hopper system with position measurements. In comparison to the Salted Kalman Filter (SKF), the algorithm presented here achieves a maximum of 63.55% reduction in estimation error magnitude over all state dimensions near impact events.

==> Old_Text/bouncingball.tex <==
% \subsection{Elastic Bouncing Ball}

% Consider a simple point mass in two dimensions $(x_1,x_2)$, elastically impacting a plane with angle $\theta$, and coefficient of restitution $\alpha$.
% This system has 1 mode with a self reset.
% The continuous dynamics are:
% \begin{align}
%     \dot{x} = \begin{bmatrix}
%     \dot{x}_1,\dot{x}_2,\dot{x}_3,\dot{x}_4
%     \end{bmatrix}^T = \begin{bmatrix}
%     x_3,x_4,0,-a_g
%     \end{bmatrix}^T
% \end{align}
% where $a_g$ is the acceleration due to gravity.

% The guard for this system is:
% \begin{align}
%     g(x) = x_2\cos{\theta} - x_1\sin{\theta}
% \end{align}

% The reset dynamics for the system are:
% \begin{align}
%     x^+ = \begin{bmatrix}
%     x_1^- \\
%     x_2^- \\
%     x_3^- + \sin{\theta} (1+ \alpha) (x_4^- \cos{\theta} - x_3^-\sin{\theta}) \\
%     x_4^- - \cos{\theta} (1+ \alpha) (x_4^- \cos{\theta} - x_3^-\sin{\theta}) \\
%     \end{bmatrix}
%     \label{eq:elasticreset}
% \end{align}

% % \begin{figure}[tb]
% %     \centering
% %     \includegraphics[width = \linewidth]{BouncingBall_Elementwise.png}
% %     \caption{Simulating a 2D bouncing ball impacting the ground 4 times. The individual states of the trajectory are shown. The ground truth is shown in blue and the iLQR based estimate of the trajectory is shown in red.
% %     }
% %     \label{fig:bouncing_ball_trajectory_elements}
% % \end{figure}

% In this section we compare the errors of the proposed method with the errors of the SKF on a nominal trajectory with initial position of $[0,10]m$ and initial velocity of $[0.5,0]\frac{m}{s}$. 
% The process noise covariance was $\text{Diag}(0.1,0.1,1.0,1.0)$ and the measurement noise covariance was $0.01I$. 
% The estimator was given access only to position measurements. 

% The velocity estimates are less accurate than the position estimates, but that is to be expected as there are no direct measurements on the velocity states.

% Using the same initial conditions and noise settings, a test was run with 100 trials to determine the average error over a variety of noise conditions. The results of this trial can be seen in Fig. \ref{fig:bouncing_ball_avg_error}.

==> Old_Text/horizon.tex <==

% \subsection{Horizon update}
% When a new state and measurement are added, the first state must and measurement must be marginalized away from the problem to keep the optimization size consistent.
% When this occurs, the cost associated with the initial position (also known as the arrival cost) must be updated. There are many ways to do this, but some of the common ones are Kalman filters and sample based filters such as UKFs, particle filters, and cell filters.
% In this case, the Salted Kalman Filter (SKF) is used to update the arrival cost mean and covariance as it is known to have good performance on hybrid system state estimation \cite{kong2021salt}.
% % For a simple EKF update, the arrival cost is updated as:
% % \begin{align}
% %     x_{pre} &= f(x_k,w = 0) \\
% %     \Sigma_{pre} &= A\Sigma_k A^T + W \\
% %     S &= C\Sigma_{pre} C^T + V \\
% %     K &= \Sigma_{pre} C^T S^{-1} \\
% %     z &= y - C*x_{pre} \\
% %     x_{k+1} &= x_{pre} + Kz \\
% %     \Sigma_{k+1} &= \Sigma_{pre} -KC\Sigma_{pre}
% % \end{align}
% % Where $A$ is the Jacobian of the dynamics about the current initial point and $C$ is the measurement Jacobian.

% The seeding for the optimization is generated by using the solution from the prior window for the first N-1 timesteps, and the final timestep is the propagation of the prior final estimate with no process noise.

% \begin{figure}[tb]
%     \centering
%     \includegraphics[width = \linewidth]{BallBounceError.jpg}
%     \caption{Average error for each state over 100 trials when simulating a bouncing ball which impacts the ground XX times during its execution. The errors from the proposed method is shown in blue solid lines while the errors from the salted Kalman filter is shown in dashed red lines.
%     }
%     \label{fig:bouncing_ball_avg_error}
% \end{figure}
